The initial state of heavy-ion collisions

We present a brief review of recent theoretical developments and related phenomenological approaches for understanding the initial state of heavy-ion collisions, with emphasis on the Color Glass Condensate formalism.

==> Figures/IniStateAA.tex <==
\subsubsection{The initial state in A+A collisions}

The CGC formalism also offers a framework which allows one to
determine the initial state of a heavy-ion collision. This refers to
the distribution of produced particles in momentum as well as
transverse coordinate space which determines the initial condition for
the subsequent thermalization stage, followed by (viscous)
hydrodynamics. Understanding the thermalization process in high-energy
heavy-ion collisions is a topic which is currently under intense
investigation; we refer the interested reader to a recent review by F.~Gelis
published in this journal~\cite{Gelis:2012ri}.

In practice, the ``detailed'' dynamics of thermalization is often
skipped and the $p_T$-integrated distribution of produced particles in
the transverse plane is used directly to initialize hydrodynamic
simulations. This appears reasonable if one is interested mainly in
the features of $dN/dyd^2r_T$ over length scales larger than the
thermalization time $\tau_{\rm th}$. On the other hand, density
fluctuations on shorter scales could be washed out, see e.g.\
ref.~\cite{Schenke:2012hg} for a concrete example applying classical
Yang-Mills field dynamics.

Instead of resorting to the CGC formalism a much simpler shortcut to
the initial $dN/dyd^2r_T$ is to assume that the local density of
particles produced at a point $r_T$ is simply proportional to the
average density of projectile and target participants, $dN/dyd^2r_T
\sim (\rho_{\rm part}^A(r_T) + \rho_{\rm part}^B(r_T))/2$. This
``wounded nucleon'' model, often times also labeled ``Glauber model'',
clearly must capture the rough features of $dN/dyd^2r_T$. On the other
hand, it is evident from the increase of $(1/N_{\rm part})\; dN/d\eta$ or
$(1/N_{\rm part})\; dE_T/d\eta$ from peripheral to central Pb+Pb
collisions by about a factor of two (see
fig.\ref{fig:PbPb_Centrality}) that such a model is far from accurate.
There is no reason to believe that the second harmonic moment of the
density distribution in the transverse plane, the so-called
eccentricity $\varepsilon = \langle y^{2}{-}x^{2}\rangle/ \langle
y^{2}{+}x^{2}\rangle$ would do better (the same goes for higher
moments). Indeed, a variety of CGC models which do describe the
centrality dependence of $dN/dy$ predict higher eccentricity
$\varepsilon$ than the ``wounded nucleon model''
\cite{Hirano:2005xf,Drescher:2006pi,Drescher:2007cd,Drescher:2006ca,Schenke:2012hg}.

The ``wounded nucleon model'' for soft particle production can be
improved by adding a semi-hard component. It has to incorporate
impact parameter and $Q^2$ dependent shadowing in order to smoothly
interpolate to p+p collisions in very peripheral collisions and to
$\sim N_{\rm coll}$ scaling at high $p_T$~\cite{Helenius:2012wd};
also, the energy dependence of the low-$p_T$ cutoff required by
leading-twist calculations needs to be fixed carefully to reproduce
measured multiplicities.

The initial spatial particle distribution exhibits large
fluctuations. They manifest in non-zero elliptic flow $v_2$ in central
heavy-ion collisions~\cite{Alver:2006wh} as well as in a large
``triangular flow'' component $v_3$~\cite{Alver:2010gr}. One source
of fluctuations is due to the locations of participant
nucleons~\cite{Alver:2006wh}; these have also been incorporated early
on in Monte-Carlo implementations of the $k_T$-factorization formula
with KLN UGDs~\cite{Drescher:2006ca,Drescher:2007ax}.

However, even for a fixed (local) number of participants there are
intrinsic particle production fluctuations. This is most evident from
the wide multiplicity distribution in non-single diffractive p+p
collisions (see section on multiplicity fluctuations). A suitable
extrapolation to A+A collisions has to be included both in ``wounded
nucleon''~\cite{Qin:2010pf} as well as in CGC
based~\cite{Dumitru:2012yr} Monte-Carlo models.  In the CGC approach,
intrinsic particle production fluctuations are expected to occur on
sub-nucleon distance scales on the order of
$\sim1/Q_s$~\cite{Schenke:2012wb}, as shown in
fig.~\ref{fig:flucsAA}. It is interesting to note that early CGC initial
state models which do {\em not} incorporate intrinsic particle
production fluctuations~\cite{Drescher:2006ca,Drescher:2007ax} appear
to be inconsistent with the distributions of angular flow harmonics
measured by the ATLAS collaboration~\cite{Jia:2012ve} while recent
approaches can describe higher eccentricity harmonics rather
well~\cite{Gale:2012rq}.
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.49\textwidth]{Figures/eps-fine-intermediate.eps}
\includegraphics[width=0.49\textwidth]{Figures/vnenDist-20-25.eps}
\end{center}
%\vspace*{-0.6cm}
\caption[a]{Left: fluctuating energy density distribution at
  midrapidity and time $\tau=0.2$~fm/c in an A+A
  collision~\cite{Schenke:2012wb}.
Right: Scaled distributions of various azimuthal harmonics for Pb+Pb
collisions at 2.76~TeV (20\%-25\% centrality class) from the CGC
implementation of ref.~\cite{Gale:2012rq} compared to ATLAS data.
}
\label{fig:flucsAA}
\end{figure}
The ``cosmology of heavy-ion collisions'' will be to understand the
nature, scale, magnitude and evolution of these fundamental QCD
fluctuations in detail. It represents a very exciting avenue for
future research.

